Observational constraints on the cosmological expansion rate and spatial curvature

Observations conducted over the last few decades show that the expansion of the Universe is accelerating. In the standard model of cosmology, this accelerated expansion is attributed to a dark energy in the form of a cosmological constant. It is conceivable, however, for the dark energy to exhibit mild dynamics (so that its energy density changes with time rather than having a constant value), or for the accelerated expansion of the Universe to be caused by some mechanism other than dark energy. In this work I will investigate both of these possibilities by using observational data to place constraints on the parameters of simple models of dynamical dark energy as well as cosmological models without dark energy. I find that these data favor the standard model while leaving some room for dynamical dark energy. The standard model also holds that the Universe is flat on large spatial scales. The same observational data used to test dark energy dynamics can be used to constrain the large-scale curvature of the Universe, and these data generally favor spatial flatness, with some mild preference for spatial curvature in some data combinations.

==> dedication.tex <==
% +--------------------------------------------------------------------+
% | Dedication Page (Optional)
% +--------------------------------------------------------------------+

\newpage
\vspace*{0.9cm}
\begin{center}
{\bf \Huge Dedication}
\end{center}

\setlength{\baselineskip}{0.8cm}

%\pdfbookmark[0]{Dedication}{PDF_Dedication}

% +--------------------------------------------------------------------+
% | Enter the text for your dedication in the space below this box.    
% +--------------------------------------------------------------------+

For my parents.


==> preface.tex <==
% +--------------------------------------------------------------------+
% | Preface (Optional)
% +--------------------------------------------------------------------+

\newpage
\vspace*{0.9cm}
\begin{center}
{\bf \Huge Preface}
\end{center}

\setlength{\baselineskip}{0.8cm}

%\pdfbookmark[0]{Preface}{PDF_Preface}

% +--------------------------------------------------------------------+
% | Enter text of your Preface in the space below this box.            
% +--------------------------------------------------------------------+

Enter the text for your Preface page in the preface.tex file. The Preface page is optional.  If you wish to remove it, see the comments in the etdrtemplate.tex file.

